From Heuristic to Analytic: Cognitively Motivated Strategies for Coherent Physical Commonsense Reasoning

Pre-trained language models (PLMs) have shown impressive performance in various language tasks. However, they are prone to spurious correlations, and often generate illusory information. In real-world applications, PLMs should justify decisions with formalized, coherent reasoning chains, but this challenge remains under-explored. Cognitive psychology theorizes that humans are capable of utilizing fast and intuitive heuristic thinking to make decisions based on past experience, then rationalizing the decisions through slower and deliberative analytic reasoning. We incorporate these interlinked dual processes in fine-tuning and in-context learning with PLMs, applying them to two language understanding tasks that require coherent physical commonsense reasoning. We show that our proposed Heuristic-Analytic Reasoning (HAR) strategies drastically improve the coherence of rationalizations for model decisions, yielding state-of-the-art results on Tiered Reasoning for Intuitive Physics (TRIP). We also find that this improved coherence is a direct result of more faithful attention to relevant language context in each step of reasoning. Our findings suggest that human-like reasoning strategies can effectively improve the coherence and reliability of PLM reasoning.

==> figures/prompt-har-pc-propara.tex <==
\begin{figure*}
\begin{mybox}{Tiered-ProPara - CICL-HAR - Conversion Story Selection}
{\normalsize \textbf{Demonstration Prompts (1 of 4):}}\\
\footnotesize
Story A: \\
1. Wind and water erode rocks.\\
2. The wind and water pick up sediment that came off the rocks.\\
3. Sediment is carried to an area by the wind, water, air, or ice.\\
4. Sediment is deposited on the same spot many times.\\
5. The sediment piles on top of other sediment for a long time.\\
6. The sediment near the bottom is compressed by the weight of newer sediment.\\
7. The sediment becomes sedimentary rock as it is pushed together by the heavy weight.\\
Story B: \\
1. Waves hit the coast.\\
2. Waves have energy that pushes the water and sediment.\\
3. The sediment can help erode land like sandpaper.\\
4. Water washes the sediment back.\\
5. Some sediment is left as sand.\\
What happened to sediment?\\
Sediment is converted in story A.\\
\\
{\normalsize \textbf{Test Prompt:}}\\
\footnotesize
Story A: \\
1. Coal is heated in the boiler.\\
2. The water tank over the boiler is heated.\\
3. Creates steam.\\
4. The steam is funneled to the piston.\\
5. Piston uses the steam as energy.\\
6. The piston causes the crankshaft to move.\\
Story B: \\
1. Plants obtain water through the soil they are growing in.\\
2. The plants roots absorb the water from the soil.\\
3. Transport the water to the parts of the plant where the water is needed.\\
4. The plant uses the water as part of the photosynthesis process.\\
5. The plant creates food, called glucose, for itself.\\
6. The plant uses water to circulate the glucose around the plant to deliver the glucose to where it's needed.\\
What happened to water?\\
\\
{\normalsize \textbf{LLM Sample Output:}} \\
\footnotesize
\textit{Water is converted in story A.\\}

\end{mybox}
\caption{Sample prompt used for conversion story selection step of prompt-chaining for in-context learning with heuristic-analytic reasoning (CICL-HAR) on Tiered-ProPara. Some redundant sections of the prompt are omitted (indicated with ``...'' and in section headings).}
\end{figure*}

\begin{figure*}
\begin{mybox}{Tiered-ProPara - CICL-HAR - Conversion Sentence Selection}

{\normalsize \textbf{Demonstration Prompts (1 of 4):}}\\
\footnotesize
Story: \\
1. Wind and water erode rocks.\\
2. The wind and water pick up sediment that came off the rocks.\\
3. Sediment is carried to an area by the wind, water, air, or ice.\\
4. Sediment is deposited on the same spot many times.\\
5. The sediment piles on top of other sediment for a long time.\\
6. The sediment near the bottom is compressed by the weight of newer sediment.\\
7. The sediment becomes sedimentary rock as it is pushed together by the heavy weight.\\
Sediment is converted in sentence 7.\\
\\
{\normalsize \textbf{Test Prompt:}}\\
\footnotesize
Story: \\
1. Coal is heated in the boiler.\\
2. The water tank over the boiler is heated.\\
3. Creates steam.\\
4. The steam is funneled to the piston.\\
5. Piston uses the steam as energy.\\
6. The piston causes the crankshaft to move.\\
What happened to water?\\

{\normalsize \textbf{LLM Sample Output:}} \\
\footnotesize
\textit{Water is converted in sentence 3.\\}
\\

\end{mybox}
\caption{Sample prompt used for conversion sentence selection step of prompt-chaining for in-context learning with heuristic-analytic reasoning (CICL-HAR) on Tiered-ProPara. Some redundant sections of the prompt are omitted (indicated with ``...'' and in section headings).}
\end{figure*}

\begin{figure*}
\begin{mybox}{Tiered-ProPara - CICL-HAR - Physical State Prediction}
{\normalsize \textbf{Demonstration Prompts (1 of 4):}}\\
\footnotesize
The sediment becomes sedimentary rock as it is pushed together by the heavy weight. What happened to sediment?\\
Sediment is converted to sedimentary rock.\\
\\
{\normalsize \textbf{Test Prompt:}}\\
\footnotesize
Creates steam. What happened to water?\\
\\
{\normalsize \textbf{LLM Sample Output:}} \\
\footnotesize
\textit{Water is converted to steam.\\}

\end{mybox}
\caption{Sample prompt used for conversion entity prediction step of prompt-chaining for in-context learning with heuristic-analytic reasoning (CICL-HAR) on Tiered-ProPara. Some redundant sections of the prompt are omitted (indicated with ``...'' and in section headings).}
\end{figure*}


==> figures/prompt-har-pc-trip.tex <==
\begin{figure*}
\begin{mybox}{TRIP - HAR-PC - Plausible Story Selection}
{\normalsize \textbf{Demonstration Prompts (1 of 4):}}\\
\footnotesize
Story A: \\
1. Mary went to the fridge.\\
2. Mary took out a bowl from the fridge.\\
3. The bowl had a cucumber and a donut in it.\\
4. Mary put the cucumber on a plate and tossed the donut in the trash.\\
5. Mary ate the donut.\\
Story B: \\
1. Mary went to the fridge.\\
2. Mary took out a bowl from the fridge.\\
3. The bowl had a cucumber and a donut in it.\\
4. Mary put the cucumber on the counter.\\
5. Mary ate the donut.\\
Story B is more plausible.\\
\\
{\normalsize \textbf{Test Prompt:}}\\
\footnotesize
Story A: \\
1. Ann opened the toolbox and realized that someone took away all of her tools.\\
2. Ann took out an axe, a pair of scissors, rope and a few other things.\\
3. Ann put these items in a box and placed them in the trunk of her car.\\
4. Ann fastened her bicycle to the bicycle rack on her car.\\
5. Ann went inside the house to get the rest of her gear to put in the car.\\
Story B: \\
1. Ann opened the toolbox to get a few things for her camping trip.\\
2. Ann took out an axe, a pair of scissors, rope and a few other things.\\
3. Ann put these items in a box and placed them in the trunk of her car.\\
4. Ann fastened her bicycle to the bicycle rack on her car.\\
5. Ann went inside the house to get the rest of her gear to put in the car.\\

{\normalsize \textbf{LLM:}}\\
\footnotesize
\textit{Story B is more plausible.\\}
\\
\end{mybox}
\caption{Sample prompt used for plausible story selection step of prompt-chaining for in-context learning with heuristic-analytic reasoning (CICL-HAR) on TRIP. Some redundant sections of the prompt are omitted (indicated with ``...'' and in section headings).}
\end{figure*}

\begin{figure*}
\begin{mybox}{TRIP - HAR-PC - Conflicting Sentence Selection}
{\normalsize \textbf{Demonstration Prompts (1 of 4):}}\\
Story: \\
1. Mary went to the fridge.\\
2. Mary took out a bowl from the fridge.\\
3. The bowl had a cucumber and a donut in it.\\
4. Mary put the cucumber on a plate and tossed the donut in the trash.\\
5. Mary ate the donut.\\
Sentences 4 and 5 conflict with each other.\\
\\
{\normalsize \textbf{Test Prompt:}}\\
\footnotesize
Story: \\
1. Ann opened the toolbox and realized that someone took away all of her tools.\\
2. Ann took out an axe, a pair of scissors, rope and a few other things.\\
3. Ann put these items in a box and placed them in the trunk of her car.\\
4. Ann fastened her bicycle to the bicycle rack on her car.\\
5. Ann went inside the house to get the rest of her gear to put in the car.\\
\\
{\normalsize \textbf{LLM:}}\\
\footnotesize
\textit{Sentences 1 and 2 conflict with each other.}\\
\\
\end{mybox}
\caption{Sample prompt used for conflicting sentence selection step of prompt-chaining for in-context learning with heuristic-analytic reasoning (CICL-HAR) on TRIP. Some redundant sections of the prompt are omitted (indicated with ``...'' and in section headings).}
\end{figure*}

\begin{figure*}
\begin{mybox}{TRIP - HAR-PC - Physical State Prediction}
{\normalsize \textbf{Demonstration Prompts - Physical States Pre-condition (3 of 40):}}\\
\footnotesize
Physical state options: no longer existent, broken, in pieces, turned off, inedible, unpowered\\
After Tom unplugged the microwave, what is the state of the microwave? The microwave is now unpowered.\\
After Tom threw the cereal in the dustbin, what is the state of the cereal? The cereal is now inedible.\\
After Tom mashed the banana, what is the state of the banana? The banana is now in pieces.\\
\\
{\normalsize \textbf{Test Prompt:}}\\
\footnotesize
After Ann opened the toolbox and realized that someone took away all of her tools, what are the state of the tools?\\

{\normalsize \textbf{LLM:}}\\
\footnotesize
\textit{The tools are now no longer existent.\\}

{\normalsize \textbf{Demonstration Prompts - Physical States Pre-condition (3 of 40):}}\\
\footnotesize
Physical state options: existent, functional, whole, turned on, edible, powered\\
Before Tom turned on the microwave, what was the state of the microwave? The microwave was powered.\\
Before Tom ate the cereal, what was the state of the cereal? The cereal was edible.\\
Before Tom cut the banana into slices, what was the state of the banana? The banana was whole.\\
\\
{\normalsize \textbf{Test Prompt:}}\\
\footnotesize
Before Ann took out an axe, a pair of scissors, rope and a few other things, what were the state of the things? \\

{\normalsize \textbf{LLM:}}\\
\footnotesize
\textit{The things were existent.\\}
\end{mybox}
\caption{Sample prompt used for physical state prediction step of prompt-chaining for in-context learning with heuristic-analytic reasoning (CICL-HAR) on TRIP. Some redundant sections of the prompt are omitted (indicated with ``...'' and in section headings).}

\end{figure*}

